Reasoning-Enhanced Healthcare Predictions with Knowledge Graph Community Retrieval

Large language models (LLMs) have demonstrated significant potential in clinical decision support. Yet LLMs still suffer from hallucinations and lack fine-grained contextual medical knowledge, limiting their high-stake healthcare applications such as clinical diagnosis. Traditional retrieval-augmented generation (RAG) methods attempt to address these limitations but frequently retrieve sparse or irrelevant information, undermining prediction accuracy. We introduce KARE, a novel framework that integrates knowledge graph (KG) community-level retrieval with LLM reasoning to enhance healthcare predictions. KARE constructs a comprehensive multi-source KG by integrating biomedical databases, clinical literature, and LLM-generated insights, and organizes it using hierarchical graph community detection and summarization for precise and contextually relevant information retrieval. Our key innovations include: (1) a dense medical knowledge structuring approach enabling accurate retrieval of relevant information; (2) a dynamic knowledge retrieval mechanism that enriches patient contexts with focused, multi-faceted medical insights; and (3) a reasoning-enhanced prediction framework that leverages these enriched contexts to produce both accurate and interpretable clinical predictions. Extensive experiments demonstrate that KARE outperforms leading models by up to 10.8-15.0% on MIMIC-III and 12.6-12.7% on MIMIC-IV for mortality and readmission predictions. In addition to its impressive prediction accuracy, our framework leverages the reasoning capabilities of LLMs, enhancing the trustworthiness of clinical predictions.

==> figures/dgra_alg.tex <==
\begin{wrapfigure}{r}{0.6\textwidth}
    % \vspace{-1em}
    \vspace{-2.5em}
    \begin{minipage}{0.6\textwidth}
        \begin{algorithm}[H]
            \caption{Dynamic Graph Retrieval and Augmentation}
            \label{alg:summary_selection}
            \KwIn{Set of communities $\mathcal{C}$, patient graph $G_p$, base context $\mathcal{B}_p$, desired number of summaries $N$}
            \KwOut{Augmented patient context $\mathcal{A}_p$}
            
            Initialize $S_p \leftarrow \emptyset$\
            
            Initialize hit counts $H(v) \leftarrow 0$ for each node $v \in V_{G_p}^{\text{direct}}$\;
            
            \While{$|S_p| < N$}{
                Compute $\text{Relevance}(C_k)$ for all $C_k \in \mathcal{C}$ using Eq.~\ref{eq:combined_relevance}\\
                Select $C_{\text{best}} \leftarrow \arg\max_{C_k \in \mathcal{C}} \text{Relevance}(C_k)$\\
                Add $S_{C_{\text{best}}}$ to $S_p$: $S_p \leftarrow S_p \cup S_{C_{\text{best}}}$\\
                For each $v \in V_{C_{\text{best}}} \cap V_{G_p}^{\text{direct}}$, $H(v) \leftarrow H(v) + 1$\\
                Remove $C_{\text{best}}$ from $\mathcal{C}$: $\mathcal{C} \leftarrow \mathcal{C} \setminus C_{\text{best}}$
            }            
            Augment patient context: $\mathcal{A}_p = \mathcal{B}_p \oplus S_p$\;
            
            \Return $\mathcal{A}_p$\;
        \end{algorithm}
    \end{minipage}
    \vspace{-3em}
\end{wrapfigure}


==> figures/kg_study.tex <==
\begin{wrapfigure}{r}{6.4cm}
  \vspace{-4.5ex}
        % \centering
        \includegraphics[width=0.47\textwidth]{figures/kg_study_.pdf}
    \vspace{-2.0em}
    \caption{Ablation study of the KG used as the knowledge source.}
    \label{fig:kg_study}
    \vspace{-3em}
\end{wrapfigure}


==> figures/metric_study.tex <==
\begin{wrapfigure}{r}{8cm}
  \vspace{-1em}
        % \centering
        \includegraphics[width=0.585\textwidth]{figures/metric_study_.pdf}
    \vspace{-2.5em}
    \caption{Ablation study of the metrics we proposed for context augmentation. Task: MIMIC-IV-Readmission.}
    \label{fig:metric_study}
    \vspace{-1em}
\end{wrapfigure}


==> figures/reasoning_chains_perf.tex <==
\begin{wrapfigure}{r}{0.35\textwidth}
\centering
\vspace{-1em}
\includegraphics[width=0.35\textwidth]{figures/reasoning_num_vs_perf.pdf}
\vspace{-2em}
\caption{\small Performance of the fine-tuned \textsc{KARE} model by the number of reasoning chains per reference patient used for training}
\label{fig:reasoning_chains_perf}
\vspace{-3em}
\end{wrapfigure}

==> tables/baseline_compare_mimic4.tex <==
\begin{table}[!h]
\caption{Mortality and readmission prediction on MIMIC-IV Dataset.
}
\centering
\resizebox{\textwidth}{!}{
\begin{threeparttable}
\begin{tabular}{llcccccccc}
\toprule 
&
& \multicolumn{4}{c}{\textbf{Mortality Prediction} $(p=21.52\%)$}
& \multicolumn{4}{c}{\textbf{Readmission Prediction} $(p=50.00\%)$}
\\
\cmidrule(lr){3-6} \cmidrule(lr){7-10} 
\textbf{Type} & \textbf{Models}   & \textbf{Accuracy}     & \textbf{Macro F1}  &\textbf{Sensitivity} &\textbf{Specificity}   & \textbf{Accuracy}     & \textbf{Macro F1} &\textbf{Sensitivity} &\textbf{Specificity}\\
\midrule
\multirow{8}{*}{ML}  &GRU \citep{chung2014empirical} &88.7 &76.4 &42.9 &99.6 &62.4 &62.2 &68.3 &56.2\\
&Transformer \citep{vaswani2017attention} &83.2 &67.9 &37.0 &94.1 &61.3 &61.3 &63.0 &59.5 \\
&RETAIN \citep{choi2016retain} &84.8 &73.8 &52.4 &92.5 &62.8 &62.6 &68.7 &56.6\\
&GRAM \citep{choi2017gram} &86.4 &74.4 &50.6 &93.7 &62.5 &62.5 &67.4 &57.8\\
&Deepr \citep{nguyen2016mathtt} &89.2 &78.9 &50.8 &98.2 &59.2 &59.2 &57.0 &61.5\\
&AdaCare \citep{ma2020adacare}  &88.7 &78.2 &50.3 &97.9 &62.9 &62.9 &58.4 &67.7\\
&GRASP \citep{zhang2021grasp} &89.9 &79.1 &47.6 &99.9 &59.7 &59.6 &53.1 &66.7 \\
&StageNet \citep{gao2020stagenet}  &88.1 &77.8 &51.9 &96.7 &62.8 &62.7 &62.6 &62.9\\
\midrule
\multirow{3}{*}{LM+ML}
&GraphCare \citep{jiang2023graphcare} \\
&RAM-EHR \citep{xu2024ramehrretrievalaugmentationmeets} \\
&EMERGE \citep{zhu2024emerge} \\
\midrule
\multirow{10}{*}{LLM} &Zero-shot (LLM: Sonnet-3.5) \\
& \quad w/ EHR context only  \\
& \quad w/ Classic RAG \\
& \quad w/ \textsc{KARE}-augmented context \\
\cmidrule(lr){2-10}
& Few-Shot (LLM: Sonnet-3.5)\\
& \quad w/ exemplar only (N=2) \\
& \quad w/ exemplar only (N=4) \\
& \quad w/ EHR-CoAgent \citep{cui2024llms}\\
& \quad w/ \textsc{KARE}-augmented context \\


\cmidrule(lr){2-10}
& \textsc{KARE} (ours)  \\



\bottomrule
\end{tabular}
% \begin{tablenotes}[flushleft]\footnotesize
% \item ${\text{[a]}}$ We retrieve up to ten documents from 30 M PubMed abstracts that are most similar to the base context. Dense retrieval is applied with Nomic \citep{nussbaum2024nomic} (dim=768).
% \item ${\text{[b]}}$ Context is augmented as described in Section \ref{subsec:patient_context} using our constructed KG communities. Up to ten community summaries are appended as supplementary information.
% \item ${\text{[c]}}$ N=2 means we retrieve two most similar patients (one from positive and the other from negative samples), similar to the strategy introduced in \citep{cui2024llms}.
% \end{tablenotes}
\end{threeparttable}
}
\vspace{-1em}
\label{tb:baseline_compare}
\end{table}


==> tables/baseline_compare_new.tex <==
\begin{table}[!t]
\vspace{-1em}
\caption{\small Comparative analysis of mortality and readmission predictions using MIMIC-III and MIMIC-IV datasets. "pos" indicates the proportion of positive samples (label = 1) in the test set. Metrics like Macro F1 and Sensitivity are emphasized by an asterisk ($^{*}$) due to their importance for handling imbalanced datasets. Results are averaged by multiple runs: 30 for ML-based, 10 for LM+ML-based, and 3 for LLM-based methods with different random seeds. We \textbf{highlight} the highest value for each metric.
}
\centering
\resizebox{\textwidth}{!}{
\begin{threeparttable}
\begin{tabular}{llcccccc}
\toprule 
&&\multicolumn{6}{c}{\textbf{MIMIC-III}}\\
&
& \multicolumn{3}{c}{\textbf{Mortality Prediction} $(\text{pos}=5.42\%)$}
& \multicolumn{3}{c}{\textbf{Readmission Prediction} $(\text{pos}=54.82\%)$}
\\
\cmidrule(lr){3-5} \cmidrule(lr){6-8} 
\textbf{Type} & \textbf{Models}   & \textbf{Accuracy}     &\textbf{Macro F1$^{*}$}  &\textbf{Sensitivity/Specificity$^{*}$}  & \textbf{Accuracy}     & \textbf{Macro F1} &\textbf{Sensitivity/Specificity}\\
\midrule
\multirow{11}{*}{ML}  &GRU \citep{chung2014empirical} &92.7 &50.7 &3.7/97.8  &62.2 &61.5 &68.9/54.0\\
&Transformer \citep{vaswani2017attention} &92.7 &51.9 &5.6/97.6  &58.8 &58.2 &65.0/51.3\\
&RETAIN \citep{choi2016retain} &92.4 &50.6 &3.7/97.6  &59.1 &56.9 &74.9/40.0\\
&GRAM \citep{choi2017gram} &92.4 &50.2 &5.2/95.2  &61.8 &60.4 &74.9/46.4 \\
&Deepr \citep{nguyen2016mathtt} &91.9 &51.0 &3.7/98.2  &62.6 &62.1 &66.7/57.6\\
&TCN \citep{bai2018empirical} &91.6 &53.2 &9.3/96.4  &63.4 &62.7 &70.7/54.7\\
&ConCare \citep{ma2020concare} &94.6 &48.6 &0.0/\textbf{100.0}  &59.2 &59.0 &61.5/56.4\\
&AdaCare \citep{ma2020adacare} &90.6 &54.1 &9.1/97.6  &61.6 &60.5 &70.8/50.3\\
&GRASP \citep{zhang2021grasp} &93.7 &49.9 &1.9/98.9  &61.3 &59.5 &74.9/44.8\\
&StageNet \citep{gao2020stagenet} &90.5 &50.5 &5.6/95.4  &60.5 &60.0 &65.1/54.9\\
&KerPrint \citep{yang2023kerprint} &92.4 &52.2 &9.8/94.7  &63.5 &62.1 &68.0/56.1\\
\midrule
\multirow{3}{*}{LM+ML}
&GraphCare \citep{jiang2023graphcare} &94.9 &58.3 &17.2/97.1  &65.4 &64.1 &70.3/57.8\\
&RAM-EHR \citep{xu2024ram} &94.4 &59.6 &14.8/98.9  &64.8 &63.5 &74.7/52.4\\
&EMERGE \citep{zhu2024emerge} &94.1 &57.7 &13.2/98.4  &63.7 &62.0 &68.0/55.9\\
\midrule
\multirow{11}{*}{LLM} &Zero-shot (LLM: Claude 3.5 Sonnet) \\
& \quad w/ EHR context only &89.5 &50.4 &6.4/94.4  &54.3 &35.4 &98.9/0.2 \\
& \quad w/ Classic RAG$^{\text{[a]}}$ &89.9 &51.2 &10.2/92.8  &53.2 &34.6 &91.2/1.4\\
& \quad w/ \textsc{KARE}-augmented context$^{\text{[b]}}$ &92.3 &54.6 &14.2/94.6  & 56.3 &43.8 &93.9/10.6\\
\cmidrule(lr){2-8}
& Few-Shot (LLM: Claude 3.5 Sonnet)\\
& \quad w/ exemplar only (N=2)$^{[\text{c}]}$ &88.7 &49.5 &5.6/93.4  &52.7 &42.2 &87.0/11.1\\
& \quad w/ exemplar only (N=4) &88.0 &49.2 &5.6/92.7  &53.6 &44.7 &84.0/15.7\\
& \quad w/ EHR-CoAgent$^{\text{[d]}}$ \citep{cui2024llms} &87.4 &51.7 &13.0/91.8  &55.2 &46.1 &78.2/20.1\\
& \quad w/ \textsc{KARE}-augmented context &91.5 &53.5 &13.7/94.0  &57.1 &49.3 &75.5/27.2\\ 

\cmidrule(lr){2-8}
& \textbf{KARE} (ours)  &\textbf{95.3} &\textbf{64.6} &\textbf{24.7}/98.3  &\textbf{73.9} &\textbf{73.7} &\textbf{76.7/70.7}\\



\bottomrule
\\
\midrule
&&\multicolumn{6}{c}{\textbf{MIMIC-IV}}\\
&
& \multicolumn{3}{c}{\textbf{Mortality Prediction} $(\text{pos}=19.16\%)$}
& \multicolumn{3}{c}{\textbf{Readmission Prediction} $(\text{pos}=46.50\%)$}
\\
\cmidrule(lr){3-5} \cmidrule(lr){6-8} 
\textbf{Type} & \textbf{Models}   & \textbf{Accuracy}     & \textbf{Macro F1$^{*}$}  &\textbf{Sensitivity/Specificity$^{*}$}  & \textbf{Accuracy}     & \textbf{Macro F1} &\textbf{Sensitivity/Specificity}\\
\midrule
\multirow{11}{*}{ML}  &GRU \citep{chung2014empirical} &88.7 &76.4 &42.9/99.6  &62.4 &62.2 &68.3/56.2\\
&Transformer \citep{vaswani2017attention} &83.7 &71.3 &47.1/92.3  &61.3 &61.3 &63.0/59.5 \\
&RETAIN \citep{choi2016retain} &84.8 &73.8 &52.4/92.4  &62.8 &62.6 &68.7/56.6\\
&GRAM \citep{choi2017gram} &86.4 &74.4 &50.6/93.9  &62.5 &62.5 &67.4/57.8\\
&Deepr \citep{nguyen2016mathtt} &89.2 &78.9 &50.8/98.2  &59.2 &59.2 &57.0/61.5\\
&TCN \citep{bai2018empirical} &89.9 &79.2 &47.6/\textbf{99.9}  &63.6 &63.5 &72.2/56.1\\
&ConCare \citep{ma2020concare} &89.8 &78.9 &47.1/\textbf{99.9}  &59.8 &59.8 &63.5/56.6\\
&AdaCare \citep{ma2020adacare}  &88.7 &78.2 &50.3/97.8  &62.9 &62.9 &58.4/\textbf{67.7}\\
&GRASP \citep{zhang2021grasp} &89.9 &79.1 &47.6/99.8  &59.7 &59.6 &53.1/66.7 \\
&StageNet \citep{gao2020stagenet}  &88.1 &77.8 &51.9/96.7  &62.8 &62.7 &62.6/62.9\\
&KerPrint \citep{yang2023kerprint} &88.7 &79.8 &53.1/98.0  &63.5 &63.3 &67.0/60.1 \\
\midrule
\multirow{3}{*}{LM+ML}
&GraphCare \citep{jiang2023graphcare} &91.5 &80.3 &57.8/96.6  &65.7 &65.5 &66.2/65.0\\
&RAM-EHR \citep{xu2024ram} &90.5 &78.4 &52.6/97.0  &65.5  &65.5 &64.0/67.0\\
&EMERGE \citep{zhu2024emerge} &90.7 &78.3 &53.4/96.6  &63.3 &63.2 &61.5/64.9 \\
\midrule
\multirow{11}{*}{LLM} &Zero-shot (LLM: Claude 3.5 Sonnet) \\
& \quad w/ EHR context only  &80.5 &47.0  &2.7/98.7  &49.4 &45.7 &81.8/21.5\\
& \quad w/ Classic RAG$^{[\text{a}]}$ &81.0 &49.9 &8.1/94.6  &49.0 &44.2 &83.2/18.8 \\
& \quad w/ \textsc{KARE}-augmented context$^{[\text{b}]}$ &83.2 &54.3 &12.7/96.3  &52.3 &49.7 &80.6/27.7\\
\cmidrule(lr){2-8}
& Few-Shot (LLM: Claude 3.5 Sonnet)\\
& \quad w/ exemplar only (N=2)$^{[\text{c}]}$ &80.8 &46.7 &2.1/99.5  &49.3 &44.7 &84.0/19.1 \\
& \quad w/ exemplar only (N=4) &81.6 &49.9 &5.3/99.8  &49.0 &44.1 &84.3/18.2\\
& \quad w/ EHR-CoAgent$^{[\text{d}]}$ \citep{cui2024llms} &81.0 &55.5 &13.8/97.0  &51.2 &46.3 &78.4/24.0\\
& \quad w/ \textsc{KARE}-augmented context &84.5 &57.4 &15.8/97.6  &54.1 &51.9 &75.2/34.1\\ 

\cmidrule(lr){2-8}
& \textbf{KARE} (ours) &\textbf{94.1} &\textbf{90.4} &\textbf{73.2}/99.8  &\textbf{73.9} &\textbf{73.8} &\textbf{85.6}/63.7 \\



\bottomrule
\end{tabular}
\begin{tablenotes}[flushleft]\footnotesize
\item ${\text{[a]}}$ We retrieve up to ten documents from 30 M PubMed abstracts that are most similar to the base context. Dense retrieval is applied with Nomic \citep{nussbaum2024nomic} (dim=768).
\item ${\text{[b]}}$ Context is augmented as described in Section \ref{subsec:patient_context} using our constructed KG communities. Up to ten community summaries are appended as supplementary information.
\item ${\text{[c]}}$ N=2 means that we retrieve two most similar patients (one from positive and the other from negative samples), similar to the strategy introduced in \citep{cui2024llms}.
\item ${\text{[d]}}$ 
Since the code for EHR-CoAgent was not open-sourced at the time of our paper submission, we implemented it ourselves, as detailed in Appendix \ref{ap:baseline_impl}.
\end{tablenotes}
\end{threeparttable}
}
\vspace{-2em}
\label{tb:baseline_compare}
\end{table}

==> tables/perf_std.tex <==
\begin{table}[!h]
\vspace{-1.5em}
\caption{\small Comparative analysis of mortality and readmission predictions using MIMIC-III and MIMIC-IV datasets. "pos" indicates the proportion of positive samples (label = 1) in the test set. Metrics like Macro F1 and Sensitivity are emphasized by an asterisk ($^{*}$) due to their importance for handling imbalanced datasets. Results are averaged by multiple runs: 30 for ML-based, 10 for LM+ML-based, and 3 for LLM-based methods with different random seeds. We \textbf{highlight} the highest value for each metric. \nc{The standard deviation is reported in bracket for each entry.}
% \cx{for all tables, could we highlight our model using bold font, and all best performance using bold font?}
}
\centering
\resizebox{\textwidth}{!}{
\begin{threeparttable}
\begin{tabular}{llcccccccc}
\toprule 
&&\multicolumn{8}{c}{\textbf{MIMIC-III}}\\
&
& \multicolumn{4}{c}{\textbf{Mortality Prediction} $(\text{pos}=5.42\%)$}
& \multicolumn{4}{c}{\textbf{Readmission Prediction} $(\text{pos}=54.82\%)$}
\\
\cmidrule(lr){3-6} \cmidrule(lr){7-10} 
\textbf{Type} & \textbf{Models}   & \textbf{Accuracy}     &\textbf{Macro F1$^{*}$}  &\textbf{Sensitivity$^{*}$} &\textbf{Specificity}   & \textbf{Accuracy}     & \textbf{Macro F1} &\textbf{Sensitivity} &\textbf{Specificity}\\
\midrule
\multirow{11}{*}{ML}  &GRU \citep{chung2014empirical} &92.7$_\text{(0.4)}$ &50.7$_\text{(0.8)}$ &3.7$_\text{(1.7)}$ &97.8$_\text{(0.9)}$ &62.2$_\text{(0.7)}$ &61.5$_\text{(0.8)}$ &68.9$_\text{(2.2)}$ &54.0$_\text{(2.8)}$\\
&Transformer \citep{vaswani2017attention} &92.7$_\text{(0.8)}$ &51.9$_\text{(1.7)}$ &5.6$_\text{(2.2)}$ &97.6$_\text{(0.8)}$ &58.8$_\text{(0.6)}$ &58.2$_\text{(0.9)}$ &65.0$_\text{(3.4)}$ &51.3$_\text{(4.5)}$\\
&RETAIN \citep{choi2016retain} &92.4$_\text{(0.6)}$ &50.6$_\text{(1.6)}$ &3.7$_\text{(1.9)}$ &97.6$_\text{(0.7)}$ &59.1$_\text{(1.0)}$ &56.9$_\text{(1.3)}$ &74.9$_\text{(3.9)}$ &40.0$_\text{(5.2)}$\\
&GRAM \citep{choi2017gram} &92.4$_\text{(0.5)}$ &50.2$_\text{(1.2)}$ &5.2$_\text{(2.0)}$ &95.2$_\text{(1.1)}$ &61.8$_\text{(0.8)}$ &60.4$_\text{(1.1)}$ &74.9$_\text{(3.1)}$ &46.4$_\text{(4.4)}$ \\
&Deepr \citep{nguyen2016mathtt} &91.9$_\text{(0.7)}$ &51.0$_\text{(1.4)}$ &3.7$_\text{(1.8)}$ &98.2$_\text{(0.6)}$ &62.6$_\text{(0.9)}$ &62.1$_\text{(1.0)}$ &66.7$_\text{(2.8)}$ &57.6$_\text{(3.5)}$\\
&TCN \citep{bai2018empirical} &91.6$_\text{(0.8)}$ &53.2$_\text{(1.1)}$ &9.3$_\text{(2.1)}$ &96.4$_\text{(0.9)}$ &63.4$_\text{(0.8)}$ &62.7$_\text{(1.0)}$ &70.7$_\text{(3.5)}$ &54.7$_\text{(5.3)}$\\
&ConCare \citep{ma2020concare} &94.6$_\text{(0.0)}$ &48.6$_\text{(0.0)}$ &0.0$_\text{(0.0)}$ &\textbf{100.0}$_\text{(0.0)}$ &59.2$_\text{(0.6)}$ &59.0$_\text{(0.7)}$ &61.5$_\text{(2.4)}$ &56.4$_\text{(3.0)}$\\
&AdaCare \citep{ma2020adacare} &90.6$_\text{(0.9)}$ &54.1$_\text{(1.3)}$ &9.1$_\text{(2.4)}$ &97.6$_\text{(1.0)}$ &61.6$_\text{(0.7)}$ &60.5$_\text{(0.8)}$ &70.8$_\text{(2.9)}$ &50.3$_\text{(3.7)}$\\
&GRASP \citep{zhang2021grasp} &93.7$_\text{(0.4)}$ &49.9$_\text{(1.1)}$ &1.9$_\text{(1.4)}$ &98.9$_\text{(0.3)}$ &61.3$_\text{(0.6)}$ &59.5$_\text{(0.9)}$ &74.9$_\text{(3.2)}$ &44.8$_\text{(4.7)}$\\
&StageNet \citep{gao2020stagenet} &90.5$_\text{(0.8)}$ &50.5$_\text{(1.2)}$ &5.6$_\text{(2.3)}$ &95.4$_\text{(1.4)}$ &60.5$_\text{(0.8)}$ &60.0$_\text{(1.0)}$ &65.1$_\text{(3.7)}$ &54.9$_\text{(4.1)}$\\
&KerPrint \citep{yang2023kerprint} &92.4$_\text{(0.5)}$ &52.2$_\text{(1.0)}$ &9.8$_\text{(1.8)}$ &94.7$_\text{(1.1)}$ &63.5$_\text{(0.6)}$ &62.1$_\text{(0.8)}$ &68.0$_\text{(2.4)}$ &56.1$_\text{(3.3)}$\\
\midrule
\multirow{3}{*}{LM+ML} 
&GraphCare \citep{jiang2023graphcare} &94.9$_\text{(0.3)}$ &58.3$_\text{(0.7)}$ &17.2$_\text{(1.6)}$ &97.1$_\text{(0.5)}$ &65.4$_\text{(0.4)}$ &64.1$_\text{(0.5)}$ &70.3$_\text{(1.7)}$ &57.8$_\text{(2.1)}$\\
&RAM-EHR \citep{xu2024ram} &94.4$_\text{(0.4)}$ &59.6$_\text{(0.8)}$ &14.8$_\text{(2.2)}$ &98.9$_\text{(0.4)}$ &64.8$_\text{(0.5)}$ &63.5$_\text{(0.7)}$ &74.7$_\text{(2.0)}$ &52.4$_\text{(2.5)}$\\
&EMERGE \citep{zhu2024emerge} &94.1$_\text{(0.5)}$ &57.7$_\text{(1.0)}$ &13.2$_\text{(2.4)}$ &98.4$_\text{(0.5)}$  &63.7$_\text{(0.6)}$ &62.0$_\text{(0.8)}$ &68.0$_\text{(2.6)}$ &55.9$_\text{(3.1)}$\\
\midrule
\multirow{11}{*}{LLM} &Zero-shot (LLM: Claude 3.5 Sonnet) \\
& \quad w/ EHR context only &89.5$_\text{(2.8)}$ &50.4$_\text{(3.5)}$ &6.4$_\text{(4.1)}$ &94.4$_\text{(2.4)}$ &54.3$_\text{(3.2)}$ &35.4$_\text{(4.7)}$ &98.9$_\text{(1.0)}$ &0.2$_\text{(0.4)}$ \\  
& \quad w/ Classic RAG$^{\text{[a]}}$ &89.9$_\text{(2.5)}$ &51.2$_\text{(3.3)}$ &10.2$_\text{(3.9)}$ &92.8$_\text{(2.2)}$ &53.2$_\text{(3.0)}$ &34.6$_\text{(4.3)}$ &91.2$_\text{(2.1)}$ &1.4$_\text{(1.3)}$\\
& \quad w/ \textsc{KARE}-augmented context$^{\text{[b]}}$ &92.3$_\text{(1.8)}$ &54.6$_\text{(2.6)}$ &14.2$_\text{(3.1)}$ &94.6$_\text{(1.7)}$ & 56.3$_\text{(2.5)}$ &43.8$_\text{(3.4)}$ &93.9$_\text{(1.8)}$ &10.6$_\text{(2.7)}$\\
\cmidrule(lr){2-10}  
& Few-Shot (LLM: Claude 3.5 Sonnet)\\
& \quad w/ exemplar only (N=2)$^{[\text{c}]}$ &88.7$_\text{(1.4)}$ &49.5$_\text{(1.8)}$ &5.6$_\text{(2.5)}$ &93.4$_\text{(1.1)}$ &52.7$_\text{(1.9)}$ &42.2$_\text{(2.3)}$ &87.0$_\text{(2.0)}$ &11.1$_\text{(2.4)}$\\  
& \quad w/ exemplar only (N=4) &88.0$_\text{(1.2)}$ &49.2$_\text{(1.6)}$ &5.6$_\text{(2.2)}$ &92.7$_\text{(1.0)}$ &53.6$_\text{(1.7)}$ &44.7$_\text{(2.1)}$ &84.0$_\text{(1.9)}$ &15.7$_\text{(2.3)}$\\
& \quad w/ EHR-CoAgent$^{\text{[d]}}$ \citep{cui2024llms} &87.4$_\text{(1.0)}$ &51.7$_\text{(1.4)}$ &13.0$_\text{(1.9)}$  &91.8$_\text{(0.9)}$ &55.2$_\text{(1.5)}$ &46.1$_\text{(1.8)}$ &78.2$_\text{(1.6)}$ &20.1$_\text{(2.0)}$\\
& \quad w/ \textsc{KARE}-augmented context &91.5$_\text{(1.0)}$ &53.5$_\text{(1.3)}$ &13.7$_\text{(1.7)}$ &94.0$_\text{(0.9)}$ &57.1$_\text{(1.1)}$ &49.3$_\text{(1.4)}$ &75.5$_\text{(1.3)}$ &27.2$_\text{(1.6)}$\\


\cmidrule(lr){2-10}
& \textbf{KARE} (ours)  &\textbf{95.3}$_\text{(0.3)}$ &\textbf{64.6}$_\text{(0.6)}$ &\textbf{24.7}$_\text{(1.4)}$ &98.3$_\text{(0.9)}$ &\textbf{73.9}$_\text{(0.5)}$ &\textbf{73.7}$_\text{(0.7)}$ &\textbf{76.7}$_\text{(0.7)}$ &\textbf{70.7}$_\text{(0.8)}$\\



\bottomrule
\\
\midrule
&&\multicolumn{8}{c}{\textbf{MIMIC-IV}}\\
&
& \multicolumn{4}{c}{\textbf{Mortality Prediction} $(\text{pos}=19.16\%)$}
& \multicolumn{4}{c}{\textbf{Readmission Prediction} $(\text{pos}=46.50\%)$}
\\
\cmidrule(lr){3-6} \cmidrule(lr){7-10} 
\textbf{Type} & \textbf{Models}   & \textbf{Accuracy}     & \textbf{Macro F1$^{*}$}  &\textbf{Sensitivity$^{*}$} &\textbf{Specificity}   & \textbf{Accuracy}     & \textbf{Macro F1} &\textbf{Sensitivity} &\textbf{Specificity}\\
\midrule
\multirow{11}{*}{ML}  &GRU \citep{chung2014empirical} &88.7$_\text{(0.3)}$ &76.4$_\text{(0.4)}$ &42.9$_\text{(2.1)}$ &99.6$_\text{(0.3)}$ &62.4$_\text{(0.6)}$ &62.2$_\text{(0.5)}$ &68.3$_\text{(1.3)}$ &56.2$_\text{(1.7)}$\\
&Transformer \citep{vaswani2017attention} &83.7$_\text{(0.6)}$ &71.3$_\text{(0.9)}$ &47.1$_\text{(3.2)}$ &92.3$_\text{(1.5)}$ &61.3$_\text{(0.8)}$ &61.3$_\text{(0.8)}$ &63.0$_\text{(2.9)}$ &59.5$_\text{(3.0)}$ \\
&RETAIN \citep{choi2016retain} &84.8$_\text{(1.2)}$ &73.8$_\text{(1.2)}$ &52.4$_\text{(2.6)}$ &92.4$_\text{(2.0)}$ &62.8$_\text{(0.7)}$ &62.6$_\text{(0.7)}$ &68.7$_\text{(1.6)}$ &56.6$_\text{(1.8)}$\\
&GRAM \citep{choi2017gram} &86.4$_\text{(0.5)}$ &74.4$_\text{(0.7)}$ &50.6$_\text{(2.3)}$ &93.9$_\text{(1.4)}$ &62.5$_\text{(0.6)}$ &62.5$_\text{(0.6)}$ &67.4$_\text{(1.9)}$ &57.8$_\text{(2.1)}$\\
&Deepr \citep{nguyen2016mathtt} &89.2$_\text{(0.4)}$ &78.9$_\text{(0.6)}$ &50.8$_\text{(1.9)}$ &98.2$_\text{(0.8)}$ &59.2$_\text{(0.9)}$ &59.2$_\text{(0.9)}$ &57.0$_\text{(2.5)}$ &61.5$_\text{(2.6)}$\\
&TCN \citep{bai2018empirical} &89.9$_\text{(0.3)}$ &79.2$_\text{(0.5)}$ &47.6$_\text{(2.2)}$ &\textbf{99.9}$_\text{(0.1)}$ &63.6$_\text{(0.7)}$ &63.5$_\text{(0.7)}$ &72.2$_\text{(1.5)}$ &56.1$_\text{(2.0)}$\\
&ConCare \citep{ma2020concare} &89.8$_\text{(0.3)}$ &78.9$_\text{(0.5)}$ &47.1$_\text{(2.1)}$ &\textbf{99.9}$_\text{(0.1)}$ &59.8$_\text{(0.8)}$ &59.8$_\text{(0.8)}$ &63.5$_\text{(2.3)}$ &56.6$_\text{(2.4)}$\\
&AdaCare \citep{ma2020adacare}  &88.7$_\text{(0.6)}$ &78.2$_\text{(0.8)}$ &50.3$_\text{(2.4)}$ &97.8$_\text{(1.0)}$ &62.9$_\text{(0.6)}$ &62.9$_\text{(0.6)}$ &58.4$_\text{(2.8)}$ &\textbf{67.7}$_\text{(2.9)}$\\
&GRASP \citep{zhang2021grasp} &89.9$_\text{(0.4)}$ &79.1$_\text{(0.6)}$ &47.6$_\text{(2.0)}$ &99.8$_\text{(0.2)}$ &59.7$_\text{(0.9)}$ &59.6$_\text{(0.9)}$ &53.1$_\text{(3.2)}$ &66.7$_\text{(3.1)}$ \\
&StageNet \citep{gao2020stagenet}  &88.1$_\text{(0.7)}$ &77.8$_\text{(0.9)}$ &51.9$_\text{(2.6)}$ &96.7$_\text{(1.2)}$ &62.8$_\text{(0.7)}$ &62.7$_\text{(0.7)}$ &62.6$_\text{(2.4)}$ &62.9$_\text{(2.5)}$\\
&KerPrint \citep{yang2023kerprint} &88.7$_\text{(0.5)}$ &79.8$_\text{(0.7)}$ &53.1$_\text{(2.2)}$ &98.0$_\text{(0.9)}$ &63.5$_\text{(0.6)}$ &63.3$_\text{(0.6)}$ &67.0$_\text{(2.0)}$ &60.1$_\text{(2.1)}$ \\
\midrule
\multirow{3}{*}{LM+ML}
&GraphCare \citep{jiang2023graphcare} &91.5$_\text{(0.4)}$ &80.3$_\text{(0.6)}$ &57.8$_\text{(1.8)}$ &96.6$_\text{(0.8)}$ &65.7$_\text{(0.5)}$ &65.5$_\text{(0.5)}$ &66.2$_\text{(1.6)}$ &65.0$_\text{(1.7)}$\\
&RAM-EHR \citep{xu2024ram} &90.5$_\text{(0.5)}$ &78.4$_\text{(0.7)}$ &52.6$_\text{(2.1)}$ &97.0$_\text{(0.9)}$ &65.5$_\text{(0.4)}$ &65.5$_\text{(0.4)}$ &64.0$_\text{(1.8)}$ &67.0$_\text{(1.9)}$\\
&EMERGE \citep{zhu2024emerge} &90.7$_\text{(0.5)}$ &78.3$_\text{(0.7)}$ &53.4$_\text{(2.0)}$ &96.6$_\text{(0.8)}$ &63.3$_\text{(0.6)}$ &63.2$_\text{(0.6)}$ &61.5$_\text{(2.1)}$ &64.9$_\text{(2.2)}$ \\
\midrule
\multirow{11}{*}{LLM} &Zero-shot (LLM: Claude 3.5 Sonnet) \\
& \quad w/ EHR context only  &80.5$_\text{(3.4)}$ &47.0$_\text{(4.2)}$ &2.7$_\text{(4.8)}$ &98.7$_\text{(2.5)}$ &49.4$_\text{(3.8)}$ &45.7$_\text{(4.0)}$ &81.8$_\text{(2.9)}$ &21.5$_\text{(3.3)}$\\
& \quad w/ Classic RAG$^{[\text{a}]}$ &81.0$_\text{(3.2)}$ &49.9$_\text{(4.0)}$ &8.1$_\text{(4.5)}$ &94.6$_\text{(2.7)}$ &49.0$_\text{(3.6)}$ &44.2$_\text{(3.9)}$ &83.2$_\text{(2.6)}$ &18.8$_\text{(3.1)}$ \\
& \quad w/ \textsc{KARE}-augmented context$^{[\text{b}]}$ &83.2$_\text{(2.6)}$ &54.3$_\text{(3.4)}$ &12.7$_\text{(3.8)}$ &96.3$_\text{(2.0)}$ &52.3$_\text{(3.0)}$ &49.7$_\text{(3.2)}$ &80.6$_\text{(2.2)}$ &27.7$_\text{(2.5)}$\\
\cmidrule(lr){2-10}
& Few-Shot (LLM: Claude 3.5 Sonnet)\\
& \quad w/ exemplar only (N=2)$^{[\text{c}]}$ &80.8$_\text{(2.0)}$ &46.7$_\text{(2.7)}$ &2.1$_\text{(3.4)}$ &99.5$_\text{(1.3)}$ &49.3$_\text{(2.4)}$ &44.7$_\text{(2.6)}$ &84.0$_\text{(1.6)}$ &19.1$_\text{(2.0)}$ \\
& \quad w/ exemplar only (N=4) &81.6$_\text{(1.8)}$ &49.9$_\text{(2.4)}$ &5.3$_\text{(3.0)}$ &99.8$_\text{(0.9)}$ &49.0$_\text{(2.2)}$ &44.1$_\text{(2.4)}$ &84.3$_\text{(1.4)}$ &18.2$_\text{(1.8)}$\\
& \quad w/ EHR-CoAgent$^{[\text{d}]}$ \citep{cui2024llms} &81.0$_\text{(1.5)}$ &55.5$_\text{(2.0)}$ &13.8$_\text{(2.6)}$ &97.0$_\text{(1.2)}$ &51.2$_\text{(1.8)}$ &46.3$_\text{(2.0)}$ &78.4$_\text{(1.2)}$ &24.0$_\text{(1.5)}$\\
& \quad w/ \textsc{KARE}-augmented context &84.5$_\text{(1.3)}$ &57.4$_\text{(1.7)}$ &15.8$_\text{(2.2)}$ &97.6$_\text{(1.0)}$ &54.1$_\text{(1.5)}$ &51.9$_\text{(1.6)}$ &75.2$_\text{(0.9)}$ &34.1$_\text{(1.2)}$\\


\cmidrule(lr){2-10}
& \textbf{KARE} (ours) &\textbf{94.1}$_\text{(0.6)}$ &\textbf{90.4}$_\text{(0.8)}$ &\textbf{73.2}$_\text{(1.3)}$ &99.8$_\text{(0.1)}$ &\textbf{73.9}$_\text{(0.4)}$ &\textbf{73.8}$_\text{(0.5)}$ &\textbf{85.6}$_\text{(0.6)}$ &63.7$_\text{(0.9)}$ \\



\bottomrule
\end{tabular}
\begin{tablenotes}[flushleft]\footnotesize
\item ${\text{[a]}}$ We retrieve up to ten documents from 30 M PubMed abstracts that are most similar to the base context. Dense retrieval is applied with Nomic \citep{nussbaum2024nomic} (dim=768).
\item ${\text{[b]}}$ Context is augmented as described in Section \ref{subsec:patient_context} using our constructed KG communities. Up to ten community summaries are appended as supplementary information.
\item ${\text{[c]}}$ N=2 means that we retrieve two most similar patients (one from positive and the other from negative samples), similar to the strategy introduced in \citep{cui2024llms}.
\item ${\text{[d]}}$ 
Since the code for EHR-CoAgent was not open-sourced at the time of our paper submission, we implemented it ourselves, as detailed in Appendix \ref{ap:baseline_impl}.
\end{tablenotes}
\end{threeparttable}
}
\vspace{-2em}
\label{tb:perf_std}
\end{table}

